Generating Origin-Destination Matrices in Neural Spatial Interaction Models

Agent-based models (ABMs) are proliferating as decision-making tools across policy areas in transportation, economics, and epidemiology. In these models, a central object of interest is the discrete origin-destination matrix which captures spatial interactions and agent trip counts between locations. Existing approaches resort to continuous approximations of this matrix and subsequent ad-hoc discretisations in order to perform ABM simulation and calibration. This impedes conditioning on partially observed summary statistics, fails to explore the multimodal matrix distribution over a discrete combinatorial support, and incurs discretisation errors. To address these challenges, we introduce a computationally efficient framework that scales linearly with the number of origin-destination pairs, operates directly on the discrete combinatorial space, and learns the agents' trip intensity through a neural differential equation that embeds spatial interactions. Our approach outperforms the prior art in terms of reconstruction error and ground truth matrix coverage, at a fraction of the computational cost. We demonstrate these benefits in large-scale spatial mobility ABMs in Cambridge, UK and Washington, DC, USA.

==> tables/metrics.tex <==
% \begin{threeparttable}
\resizebox{\textwidth}{!}{%
\begin{tabular}{
V{4.0}
m{0.16\textwidth}V{4.0}
m{0.06\textwidth}|
m{0.07\textwidth}|
>{\centering\arraybackslash}m{0.11\textwidth}|
%
>{\centering\arraybackslash}m{0.06\textwidth}
>{\centering\arraybackslash}m{0.06\textwidth}
>{\centering\arraybackslash}m{0.06\textwidth}
>{\centering\arraybackslash}m{0.06\textwidth}
>{\centering\arraybackslash}m{0.06\textwidth}V{4.0}
%
>{\centering\arraybackslash}m{0.06\textwidth}
>{\centering\arraybackslash}m{0.06\textwidth}
>{\centering\arraybackslash}m{0.06\textwidth}
>{\centering\arraybackslash}m{0.06\textwidth}
>{\centering\arraybackslash}m{0.06\textwidth}V{4.0}
}

\hlineB{4.0}
\multirow{2}{0.16\textwidth}{\textsc{Origin-Destination Matrix}} & \multirow{2}{0.06\textwidth}{$\allconstraints$} & \multirow{2}{0.07\textwidth}{$\sigma$} & \multirow{2}{0.11\textwidth}{\textsc{Quantity} $g$} & \multicolumn{5}{c V{3.0}}{\textsc{SRMSE} $\left(\expectation \left[g^{(1:N)}\right],\groundtruthtable\right)$} & \multicolumn{5}{c V{3.0}}{99\% \textsc{High Probability Region CP} $\left(g^{(1:N)}, \groundtruthtable \right)$} \\ \cline{5-14} 
 &  &  &  & \multicolumn{2}{c}{\frameworkfig}  & \multirow{2}{0.06\textwidth}{\citepalias{zachos2024}} & \multirow{2}{0.06\textwidth}{\citepalias{gaskin2023}} & \multirow{2}{0.06\textwidth}{\citepalias{ellam2018}} & \multicolumn{2}{c}{\frameworkfig} & \multirow{2}{0.06\textwidth}{\citepalias{zachos2024}} & \multirow{2}{0.06\textwidth}{\citepalias{gaskin2023}} & \multirow{2}{0.06\textwidth}{\citepalias{ellam2018}} \\
 &  &  &  & \textsc{Disjoint} & \textsc{Joint} &  &  & & \textsc{Disjoint} & \textsc{Joint} &  &  & \\ \hlineB{4.0}

 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.49 & 29.52 & 0.74 & 1.06 & 0.74 & 4\% & 2\% & 22\% & 79\% & 21\% \\
 &  & \multirow{-2}{0.07\textwidth}{$0.014$} & $\mytable\vert\allconstraints,\obsdata$ & 1.61 & 1.73 & 0.96 & $-$ & $-$ & 4\% & 1\% & 72\% & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 1.04 & 29.52 & \intensitycolour{\emph{\textbf{0.70}}} & 1.08 & \intensitycolour{\emph{\textbf{0.70}}} & 82\% & 2\% & 43\% & \intensitycolour{\emph{89\%}} & 42\% \\
 &  & \multirow{-2}{0.07\textwidth}{$0.141$} & $\mytable\vert\allconstraints,\obsdata$ & 1.61 & 1.73 & \tablecolour{ \emph{0.95}} & $-$ & $-$ & 6\% & 1\% & \tablecolour{ \emph{\textbf{94\%}}} & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.53 & 29.52 & $-$ & 1.13 & $-$ & 8\% & 2\% & $-$ & 88\% & $-$ \\
 & \multirow{-6}{0.06\textwidth}{$\myintensitytotal$} & \multirow{-2}{0.07\textwidth}{learned} & $\mytable\vert\allconstraints,\obsdata$ & 1.61 & 1.73 & $-$ & $-$ & $-$ & 4\% & 1\% & $-$ & $-$ & $-$ \\ \Xcline{2-14}{1.5pt}
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.52 & 2.52 & 0.73 & 1.06 & 0.74 & 4\% & 4\% & 21\% & 79\% & 21\% \\
 &  & \multirow{-2}{0.07\textwidth}{$0.014$} & $\mytable\vert\allconstraints,\obsdata$ & 2.52 & 2.52 & 0.73 & $-$ & $-$ & 11\% & 11\% & 67\% & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.43 & 2.43 & \intensitycolour{ \emph{\textbf{0.70}}} & 1.08 & \intensitycolour{\emph{\textbf{0.70}}} & 23\% & 24\% & 41\% & \intensitycolour{\emph{89\%}} & 42\% \\
 &  & \multirow{-2}{0.07\textwidth}{$0.141$} & $\mytable\vert\allconstraints,\obsdata$ & 2.43 & 2.43 & \tablecolour{\emph{\textbf{0.70}}} & $-$ & $-$ & 30\% & 31\% & \tablecolour{ \emph{\textbf{68\%}}} & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.52 & 2.52 & $-$ & 1.13 & $-$ & 9\% & 9\% & $-$ & 88\% & $-$ \\
\multirow{-12}{0.16\textwidth}{Total constrained} & \multirow{-6}{0.06\textwidth}{$\mytabletotal$, $\myintensitytotal$} & \multirow{-2}{0.07\textwidth}{learned} & $\mytable\vert\allconstraints,\obsdata$ & 2.52 & 2.52 & $-$ & $-$ & $-$ & 14\% & 15\% & $-$ & $-$ & $-$ \\ \Xcline{1-14}{1.5pt}
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.53 & 2.52 & 0.69 & 1.06 & 0.74 & 5\% & 5\% & 23\% & 79\% & 21\% \\
 &  & \multirow{-2}{0.07\textwidth}{$0.014$} & $\mytable\vert\allconstraints,\obsdata$ & 1.46 & 1.46 & 0.69 & $-$ & $-$ & 39\% & 39\% & 68\% & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.31 & 2.41 & \intensitycolour{\emph{\textbf{0.63}}} & 1.08 & 0.70 & 66\% & 32\% & 40\% & \intensitycolour{\emph{89\%}} & 42\% \\
 &  & \multirow{-2}{0.07\textwidth}{$0.141$} & $\mytable\vert\allconstraints,\obsdata$ & 1.19 & 1.27 & \tablecolour{ \emph{\textbf{0.63}}} & $-$ & $-$ & \tablecolour{ \emph{\textbf{94\%}}} & 73\% & 71\% & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.53 & 2.53 & $-$ & 1.13 & $-$ & 9\% & 8\% & $-$ & 88\% & $-$ \\
 & \multirow{-6}{0.06\textwidth}{$\mytablerowsums$, $\myintensitytotal$} & \multirow{-2}{0.07\textwidth}{learned} & $\mytable\vert\allconstraints,\obsdata$ & 1.48 & 1.49 & $-$ & $-$ & $-$ & 43\% & 42\% & $-$ & $-$ & $-$ \\ \Xcline{2-14}{1.5pt} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 0.58 & 0.58 & 0.69 & 0.43 & 0.69 & 53\% & 53\% & 23\% & 89\% & 23\% \\
 &  & \multirow{-2}{0.07\textwidth}{$0.014$} & $\mytable\vert\allconstraints,\obsdata$ & 0.58 & 0.58 & 0.69 & $-$ & $-$ & 82\% & 81\% & 68\% & $-$ & $-$ \\ \cline{3-14}
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 0.43 & 0.43 & 0.62 & \intensitycolour{\emph{\textbf{0.41}}} & 0.63 & 90\% & 90\% & 42\% & \intensitycolour{\emph{94\%}} & 42\% \\
 &  & \multirow{-2}{0.07\textwidth}{$0.141$} & $\mytable\vert\allconstraints,\obsdata$ & \tablecolour{ \emph{0.43}} & \tablecolour{ \emph{0.43}} & 0.61 & $-$ & $-$ & \cellcolor{gray!20}\tablecolour{ \emph{\textbf{95}\%}} & \cellcolor{gray!20}\tablecolour{ \emph{\textbf{95}\%}} & 72\% & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 0.58 & 0.58 & $-$ & 0.44 & $-$ & 73\% & 72\% & $-$ & 88\% & $-$ \\
\multirow{-12}{0.16\textwidth}{Singly constrained} & \multirow{-6}{0.06\textwidth}{$\mytablerowsums$, $\myintensitytotal$, $\myintensityrowsums$} & \multirow{-2}{0.07\textwidth}{learned} & $\mytable\vert\allconstraints,\obsdata$ & 0.58 & 0.58 & $-$ & $-$ & $-$ & 86\% & 87\% & $-$ & $-$ & $-$ \\\Xcline{1-14}{1.5pt}
 & \multicolumn{1}{l|}{} &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.52 & \intensitycolour{\emph{0.67}} & 0.71 & $-$ & $-$ & 4\% & 37\% & 21\% & $-$ & $-$ \\
 & \multicolumn{1}{l|}{} & \multirow{-2}{0.07\textwidth}{$0.014$} & $\mytable\vert\allconstraints,\obsdata$ & 1.19 & 0.59 & 0.59 & $-$ & $-$ & 61\% & 87\% & 69\% & $-$ & $-$ \\ \cline{3-14} 
 & \multicolumn{1}{l|}{} &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.50 & 0.68 & 1.22 & $-$ & $-$ & 18\% & \intensitycolour{\emph{78\%}} & 20\% & $-$ & $-$ \\
 & \multicolumn{1}{l|}{} & \multirow{-2}{0.07\textwidth}{$0.141$} & $\mytable\vert\allconstraints,\obsdata$ & 1.15 & \tablecolour{ \emph{\textbf{0.55}}} & 0.59 & $-$ & $-$ & 68\% & \tablecolour{ \emph{\textbf{89\%}}} & 86\% & $-$ & $-$ \\ \cline{3-14} 
 & \multicolumn{1}{l|}{} &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.52 & \intensitycolour{\emph{0.67}} & $-$ & $-$ & $-$ & 8\% & 49\% & $-$ & $-$ & $-$ \\
\multirow{-6}{0.16\textwidth}{Doubly constrained} & \multicolumn{1}{l|}{\multirow{-6}{0.06\textwidth}{$\mytablerowsums$, $\mytablecolsums$, $\myintensitytotal$}} & \multirow{-2}{0.07\textwidth}{learned} & $\mytable\vert\allconstraints,\obsdata$ & 1.17 & 0.59 & $-$ & $-$ & $-$ & 66\% & 86\% & $-$ & $-$ & $-$ \\ \Xcline{1-14}{1.5pt}
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.52 & 0.89 & \intensitycolour{\emph{0.71}} & $-$ & $-$ & 4\% & 49\% & 22\% & $-$ & $-$ \\
 &  & \multirow{-2}{0.07\textwidth}{$0.014$} & $\mytable\vert\allconstraints,\obsdata$ & 1.09 & \tablecolour{ \emph{\textbf{0.42}}} & 0.55 & $-$ & $-$ & 69\% & \tablecolour{ \emph{\textbf{92\%}}} & 89\% & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.50 & 0.87 & 1.10 & $-$ & $-$ & 18\% & \intensitycolour{\emph{79\%}} & 32\% & $-$ & $-$ \\
 &  & \multirow{-2}{0.07\textwidth}{$0.141$} & $\mytable\vert\allconstraints,\obsdata$ & 1.06 & 0.43 & 0.56 & $-$ & $-$ & 71\% & \tablecolour{ \emph{\textbf{92\%}}} & 88\% & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.52 & 0.89 & $-$ & $-$ & $-$ & 8\% & 51\% & $-$ & $-$ & $-$ \\
\multirow{-6}{0.16\textwidth}{Doubly and 10\% cell constrained} & \multirow{-6}{0.06\textwidth}{$\mytablerowsums$, $\mytablecolsums$, $\cellcolour{T_{\mathcal{X}_1}}$, $\myintensitytotal$} & \multirow{-2}{0.07\textwidth}{learned} & $\mytable\vert\allconstraints,\obsdata$ & 1.08 & 0.43 & $-$ & $-$ & $-$ & 70\% & \tablecolour{ \emph{\textbf{92\%}}} & $-$ & $-$ & $-$ \\ \Xcline{1-14}{1.5pt}
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.52 & 0.94 & \intensitycolour{\emph{0.71}} & $-$ & $-$ & 4\% & 42\% & 26\% & $-$ & $-$ \\
 &  & \multirow{-2}{0.07\textwidth}{$0.014$} & $\mytable\vert\allconstraints,\obsdata$ & 1.04 & 0.38 & 0.51 & $-$ & $-$ & 70\% & 92\% & 89\% & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.50 & 0.92 & 1.06 & $-$ & $-$ & 18\% & \intensitycolour{\emph{78\%}} & 32\% & $-$ & $-$ \\
 &  & \multirow{-2}{0.07\textwidth}{$0.141$} & $\mytable\vert\allconstraints,\obsdata$ & 1.02 & 0.38 & 0.51 & $-$ & $-$ & 74\% & \tablecolour{ \emph{\textbf{94\%}}} & 90\% & $-$ & $-$ \\ \cline{3-14} 
 &  &  & $\myintensity\vert\allconstraints,\obsdata$ & 2.52 & 0.96 & $-$ & $-$ & $-$ & 8\% & 47\% & $-$ & $-$ & $-$ \\
\multirow{-6}{0.16\textwidth}{Doubly and 20\% cell constrained} & \multirow{-6}{0.06\textwidth}{$\mytablerowsums$, $\mytablecolsums$, $\cellcolour{T_{\mathcal{X}_2}}$, $\myintensitytotal$} & \multirow{-2}{0.07\textwidth}{learned} & $\mytable\vert\allconstraints,\obsdata$ & 1.04 & \cellcolor{gray!20}\tablecolour{ \emph{\textbf{0.37}}} & $-$ & $-$ & $-$ & 72\% & 93\% & $-$ & $-$ & $-$ \\
 \hlineB{4.0}
\end{tabular}
}
\raggedleft{\makebox[\textwidth][r]{\fbox{$-$: This case is not handled by the approach mentioned in the column.}}}
% \fbox{%
% \hfill%
% \begin{minipage}{0.3\textwidth}\raggedright
% \hfill TEXT
% \end{minipage}}

% \begin{tablenotes}
% \item $-$ \;:  This case is incompatible with the method (column) at hand.
% \end{tablenotes}
% \end{threeparttable}

 % \colorbox{gray!20}{highlighted cells}). On an OD model basis (first column) we obtain the best reconstruction errors (SRMSE) and ground truth cell coverage probability (CP) in $\mytable$-space in all but the Total Constrained ODM model (see \tablecolour{\emph{cells}} across $\sigma$). The presence of more \tablecolour{\textbf{\emph{cells}}} than \intensitycolour{\textbf{\emph{cells}}} indicates that inference on the discrete table space offers lower SRMSE and higher CP. In loosely constrained models the MCMC method of \citep{zachos2024} outperforms ours in the $\myintensity$ space (see \intensitycolour{\emph{cells}} across $\sigma$). This is due to a limited support enforced on $\boldsymbol{\theta} \in [0,2]^2$ instead of $\reals^2$), which has a regularisation effect. In the absence of substantial $\allconstraints$ data this effect is more pronounced as it helps attain a lower error-coverage trade-off
